Scalar Communication via Random Direction Refreshing for Distributed Optimization

Distributed optimization over networks requires agents to repeatedly exchange decision variables with their neighbors. When the decision dimension $d$ is large, these exchanges dominate the communication cost, which is critical for bandwidth-constrained agents. Existing remedies quantize or sparsify the exchanged vectors, yet each message still scales with $d$ and the compression error must be compensated by additional states. To address this limitation, we propose a scalar-communication mechanism in which every neighbor message carries a single real number regardless of $d$. Agents regenerate a common random direction from a shared seed, transmit only the inner product of their state with that direction, and act on the resulting rank-one surrogate of their neighbors' states while retaining full local gradients. We develop and analyze the mechanism for an existing continuous-time distributed optimization algorithm. For strongly convex local costs with Lipschitz gradients, we show that the optimizer remains the unique consensus equilibrium, that a fixed direction admits spurious equilibria, and that refreshing the direction at a sufficiently high rate yields exponential mean-square and almost-sure convergence with constant gains and no residual error. The framework admits any isotropic fixed-norm direction distribution, including Rademacher, scaled-coordinate, and sphere-normalized Gaussian directions; all three attain lower fresh-encoding variance than unnormalized Gaussian directions. The effects of the direction distribution and the refresh interval are illustrated in~simulations.

==> Intro0.tex <==
\section{Introduction}
Distributed optimization enables a network of agents to minimize a sum of local objective functions through local computation and neighbor communication. Applications include cooperative control, distributed estimation, resource allocation, and networked learnin \cite{---}. Consensus provides a fundamental mechanism for coordinating the agents' decisions. Classical results characterize how graph connectivity and spectral properties govern agreement, while randomized gossip demonstrates how local randomized interactions can support distributed averaging~\cite{olfati2007consensus,boyd2006gossip}. For optimization, the challenge is to combine this agreement mechanism with local descent so that the common limit minimizes the aggregate objective.

Early distributed subgradient methods established convergence guarantees by combining local subgradient evaluations with information exchange over a network~\cite{nedic2009subgradient}. Subsequent methods, including EXTRA and gradient tracking, enabled exact convergence with fixed step sizes under suitable assumptions~\cite{shi2015extra,nedic2017diging}. Continuous-time coordination algorithms provide a complementary perspective in which gradient feedback, consensus coupling, and integral correction are analyzed using stability tools. In particular, Kia \emph{et al.}~\cite{kia2015continuous} developed continuous-time distributed optimization dynamics and studied their implementation with periodic and event-triggered communication. These developments motivate reducing communication while preserving local optimization capability.

Communication becomes especially demanding when the decision variable is high dimensional and neighboring agents exchange full state or update vectors. Several approaches address this limitation. Quantized consensus studies agreement when exchanged information has restricted precision~\cite{kashyap2007quantized}. In distributed learning, QSGD quantifies a tradeoff between gradient quantization and estimator variance~\cite{alistarh2017qsgd}. Sparsification communicates selected coordinates, while memory and error-feedback mechanisms retain information discarded by compression~\cite{stich2018memory,karimireddy2019error}. Quantization reduces representation precision, sparsification reduces the number of transmitted entries, and scheduling reduces transmission frequency. Their convergence properties depend on both the compressor and its integration into the underlying algorithm.


For decentralized optimization, Koloskova
\emph{et al.}~\cite{koloskova2019choco} developed algorithms in
which neighboring agents exchange quantized or sparsified model
updates, with convergence guarantees for both distributed averaging
and stochastic optimization. Their analysis accommodates biased and
unbiased compression operators. Compressed gradient tracking further
combines communication compression with local estimates of the
aggregate gradient to obtain linear convergence for smooth, strongly
convex objectives~\cite{liao2022compressed}. Robust compressed
push--pull methods extend this direction to directed networks and
nonconvex objectives while accommodating relative and absolute
compression errors~\cite{liao2024robust}.

A complementary approach reduces each transmitted vector to a scalar
through random encoding and decoding. In our recent federated
learning work, \emph{FedScalar}~\cite{rostami2024fedscalar} encodes
local model-update differences, while
\emph{ScalarFedLQR}~\cite{rostami2026scalar} encodes local
zeroth-order policy-gradient estimates. Each client transmits a
scalar inner product and a compact seed, allowing the server to
regenerate the direction and aggregate decoded update estimates.
This reduces the per-client uplink payload from $\mathcal O(d)$ to
$\mathcal O(1)$ scalar-sized quantities, independently of the model
or policy dimension $d$, and motivates applying the same communication
principle to neighbor interactions in distributed optimization.

Building on this line of research, the present paper applies random
encoding and decoding to the state vectors exchanged in
consensus-based distributed optimization. All agents regenerate a
common direction $u_k\in\mathbb R^d$ at times $t_k=k\tau$ using a
shared seed and synchronized index. Agent $i$ communicates
$c^i(t)=u_k^\top x^i(t)$, and its neighbors decode $u_kc^i(t)$ to
construct the coupling $u_ku_k^\top(x^i(t)-x^j(t))$. The local
gradient remains $\nabla f^i(x^i(t))$. Each neighbor exchange
therefore carries one real-valued component instead of a
$d$-dimensional state, reducing its dimensional cost from
$\mathcal O(d)$ to $\mathcal O(1)$ without communicating the direction
vector or introducing additional compression-error memory. Our
continuous-time model retains a continuously varying scalar signal
within each direction-holding interval; sampling and finite-bit
quantization are separate implementation considerations.

The framework admits any direction distribution satisfying
isotropy, $\mathbb E[u_ku_k^\top]=I_d$, and the stated
exponential-moment condition, with independent draws across refreshes.
Gaussian and Rademacher directions are two admissible choices,
rather than restrictions on the mechanism. Uniform coordinate
communication is also included by selecting $u_k=\sqrt d\,e_{J_k}$,
where $J_k$ is uniform on $\{1,\ldots,d\}$. This flexibility allows
the direction choice to reflect the geometry of the disagreement.
When coordinate-wise disagreement energies are approximately equal,
coordinate sampling can provide more consistent initial progress
because each selection exposes a comparable amount of disagreement.
When disagreement is concentrated in a few coordinates, many
coordinate selections miss the active components, whereas dense
Rademacher or Gaussian directions mix those components into the
transmitted scalar and can improve transient reliability. These
benefits depend on the disagreement structure and do not imply a
universal ordering of expected convergence rates. Coordinate
selection here applies to communication; local gradients remain
full dimensional.

The analysis must account for the interaction between random
communication and the coupled state and integral dynamics. Although
the encoder is unbiased at each refresh, retaining a direction over
a nonzero interval creates dependence between that direction and
the evolving network state. We control this dependence by combining
conditional Lyapunov drift at refresh times with bounds on the
intervening evolution. The resulting analysis establishes three
properties: preservation and uniqueness of the common optimal
equilibrium on the zero-sum integral-state subspace; exponential
mean-square and almost-sure convergence under an explicit sufficient
upper bound on the refresh interval, for strongly convex local
objectives with globally Lipschitz gradients and constant positive
gains; and distribution-dependent encoding-variance identities for
Gaussian, Rademacher, and scaled coordinate directions. The refresh
bound makes the roles of graph connectivity, objective regularity,
and direction statistics explicit. Under these conditions, scalar
communication preserves exact convergence to the optimizer.

\clearpage


==> communicationreduction0.tex <==
\section{Scalar communication via ...}\label{sec:scalar}
In large-scale or high-dimensional applications ($d \gg 1$), exchanging the entire $d$-dimensional vector $x^i$ between neighbors at every instant incurs substantial communication overhead. To alleviate this, we propose a scheme where all agents synchronously share a common random vector $u_k\in\mathbb{R}^d$. The vector is drawn independently of the past at times $t_k=k\tau$, with $\tau>0$, and is held constant on $[t_k,t_{k+1})$. The standard normal distribution $\mathcal{N}(0,I_d)$ is one choice; no normalization is required. A common seed, the same pseudorandom generator, and a synchronized index $k$ allow all agents to regenerate the same vector locally.

Instead of transmitting $x^i \in \mathbb{R}^d$, agent $i$ only transmits a \textbf{scalar encoding}:
\begin{equation}
    c^i(t) = u_k^\top x^i(t) \in \mathbb{R},\quad t\in[t_k,t_{k+1}).
\end{equation}
Upon receiving $c^j$ from its neighbors, agent $i$ decodes the rank-one surrogate $y^j=u_kc^j=u_ku_k^\top x^j\in\mathbb{R}^d$. This is not a reconstruction of the full state from a single scalar. The modified algorithm becomes:
\begin{align}
    \dot{v}^i &= \alpha\beta \sum\nolimits_{j=1}^N a_{ij} (y^i - y^j), \label{eq:mod_v} \\
    \dot{x}^i &= -\alpha \nabla f^i(x^i) - \beta \sum\nolimits_{j=1}^N a_{ij} (y^i - y^j) - v^i. \label{eq:mod_x}
\end{align}
The local gradient is evaluated at the actual state $x^i$; only the messages used for neighbor coupling are encoded and decoded. This reduces the communicated state dimension from $\mathcal{O}(d)$ entries to $\mathcal{O}(1)$ entry per message. In this continuous-time model, $c^i(t)$ varies continuously within each holding interval; finite-bit communication costs also depend on sampling and quantization.

\subsection{Equilibrium Analysis}
We analyze whether the true unconstrained optimizer $z^*$ of \eqref{eq:global_opt} acts as a valid equilibrium point under this modified structure. Let us denote a constant equilibrium of the state and tracking variables by $(\bar{x},\bar{v})$. The decoded variables may still change when the direction changes.

For any fixed direction, setting $\dot{v}^i=0$ in \eqref{eq:mod_v} yields:
\begin{equation}
    \sum\nolimits_{j=1}^N a_{ij}(\bar{y}^i-\bar{y}^j)=0
    \ \Longleftrightarrow\ (L\otimes I_d)\bar{y}=0,
\end{equation}
where $L$ is the graph Laplacian. Since $\mathcal{G}$ is connected, its null-space is spanned by $\mathbf{1}_N$. This guarantees consensus on the decoded variables, but does not by itself imply that $\bar{x}^i=z^*$.

To verify the desired equilibrium directly, set
\begin{equation}
    \bar{x}^i=z^*,\qquad
    \bar{v}^i=-\alpha\nabla f^i(z^*).
\end{equation}
For every shared direction $u_k$, the decoded states then satisfy
\begin{equation}
    \bar{y}^1=\cdots=\bar{y}^N=u_ku_k^\top z^*.
\end{equation}
Consequently, all neighbor differences vanish and
\begin{equation}
    \dot{v}^i=0,\qquad
    \dot{x}^i=-\alpha\nabla f^i(z^*)-\bar{v}^i=0.
\end{equation}
Because the graph is undirected, the sum of the integral variables is conserved over time:
\begin{equation}
    \sum_{i=1}^N v^i(t)=\sum_{i=1}^N v^i(0)=0.
\end{equation}
The proposed equilibrium respects this condition since
\begin{equation}
    \sum_{i=1}^N\bar{v}^i
    =-\alpha\sum_{i=1}^N\nabla f^i(z^*)=0.
\end{equation}
This is precisely the first-order necessary and sufficient condition for global optimality of $F$. Thus, \textbf{the optimal consensus state is an exact equilibrium for every shared direction}.

Moreover, if $\mathbb{E}[u_ku_k^\top]=I_d$, any constant equilibrium common to almost every direction must satisfy $(L\otimes I_d)\bar{x}=0$. Indeed, this follows by averaging $(L\otimes u_ku_k^\top)\bar{x}=0$ for that constant state. Summing the equilibrium equations for $\dot{x}^i$ then gives $\sum_i\nabla f^i(\bar{x}^i)=0$. Hence the common equilibrium on the zero-sum tracking subspace is unique.

\subsection{Why a Fixed Vector $u$ Can Fail}
While $z^*$ is a valid consensus equilibrium, choosing a static vector $u$ and holding it constant across all time need not yield convergence in dimension $d>1$.

\subsection{Geometric Incompatibility and Spurious Equilibria}
Let $P=uu^\top\in\mathbb{R}^{d\times d}$ be the rank-one encoding-decoding operator. It is an orthogonal projection only when $\|u\|=1$. The consensus term relies entirely on:
\begin{equation}
    y^i-y^j=P(x^i-x^j).
\end{equation}
If two adjacent agents have states whose difference lies in $\operatorname{span}(u)^\perp$, then:
\begin{equation}
    P(x^i-x^j)=0\quad\Longrightarrow\quad y^i-y^j=0.
\end{equation}
Consequently, the coupling is blind to disagreement in the remaining $d-1$ dimensions. A state profile is a spurious equilibrium when, in addition,
\begin{align}
    x^i-x^j&\in\operatorname{span}(u)^\perp,
       &&\forall(i,j)\in\mathcal E,\\
    v^i&=-\alpha\nabla f^i(x^i),
       &\sum_{i=1}^N\nabla f^i(x^i)&=0.
\end{align}
For example, consider two agents with $f^1(z)=\frac12\|z-a\|^2$ and $f^2(z)=\frac12\|z+a\|^2$, where $a\ne0$ and $u^\top a=0$. The global optimizer is $z^*=0$, but $x^1=a$, $x^2=-a$, and $v^1=v^2=0$ form a nonconsensus equilibrium. Thus, a fixed direction does not provide a general convergence guarantee.

\subsection{Why Dynamic Resampling Succeeds}
To remove the obstruction caused by a fixed direction, let $u_k$ be redrawn independently from a fixed distribution at the refresh times $t_k=k\tau$. The following analysis gives a sufficient upper bound on $\tau$; unbiasedness alone is not a convergence condition for arbitrary holding intervals.

Let $\mathcal F_k$ denote the history immediately before drawing $u_k$, and assume
\begin{equation}\label{eq:isotropy}
    \mathbb E[u_ku_k^\top\mid\mathcal F_k]=I_d.
\end{equation}
This holds for independent standard Gaussian vectors, independent Rademacher vectors, and $u_k=\sqrt d\,e_{J_k}$ with $J_k$ uniform on $\{1,\ldots,d\}$. The last choice gives coordinate communication as a special case.

At each refresh time, the states are determined by $\mathcal F_k$. Therefore,
\begin{align}
 &\mathbb E[y^i(t_k^+)-y^j(t_k^+)\mid\mathcal F_k]\\
 &\qquad=\mathbb E[u_ku_k^\top\mid\mathcal F_k]
          (x^i(t_k)-x^j(t_k))\nonumber\\
 &\qquad=x^i(t_k)-x^j(t_k).\nonumber
\end{align}
Within a holding interval, the states depend on the sampled direction. Hence this conditional factorization is used at the refresh times, not at every interior time. A sufficiently small holding interval allows the resulting state-direction dependence to be controlled.

Let $x=\operatorname{col}(x^1,\ldots,x^N)$, and define the stacked cost $G(x)=\sum_{i=1}^N f^i(x^i)$. Its gradient stacks the local gradients; it is distinguished from the common-argument cost $F(z)$ in \eqref{eq:global_opt}. Let
\begin{equation}
    x^*=\mathbf1_N\otimes z^*,\qquad v^*=-\alpha\nabla G(x^*),
\end{equation}
and define the error coordinates $\tilde x=x-x^*$ and $\tilde v=v-v^*$. Consider the quadratic Lyapunov candidate:
\begin{equation}\label{eq:V_original}
 V=\frac12\tilde x^\top\tilde x
    +\frac1{2\alpha\beta}\tilde v^\top
          (L^\dagger\otimes I_d)\tilde v,
\end{equation}
where $L^\dagger$ is the Moore--Penrose pseudoinverse. Since $\sum_i\tilde v^i=0$, this function is positive definite on the invariant tracking subspace.

Set $h=\nabla G(x)-\nabla G(x^*)$ and $P=u_ku_k^\top$ on the current interval. Substitution of the actual dynamics gives
\begin{align}\label{eq:actual_V_dot}
 \dot V={}&-\alpha\tilde x^\top h
       -\beta\tilde x^\top(L\otimes P)\tilde x\nonumber\\
     &+\tilde v^\top[I_N\otimes(P-I_d)]\tilde x.
\end{align}
Here the identity $\tilde v^\top(L^\dagger L\otimes P)=\tilde v^\top(I_N\otimes P)$ follows from the zero-sum condition. At a refresh time, taking conditional expectation yields
\begin{align}\label{eq:mean_V_dot}
 \mathbb E[\dot V(t_k^+)\mid\mathcal F_k]
   ={}&-\alpha\tilde x_k^\top h_k\nonumber\\
      &-\beta\tilde x_k^\top(L\otimes I_d)\tilde x_k\\
   \leq{}&-\alpha m_f\|\tilde x_k\|^2.\nonumber
\end{align}
The tracking cross terms thus cancel in this conditional expectation. For the deterministic averaged dynamics, the same calculation holds at all times. On $\{\tilde x=0\}$, invariance requires $\dot{\tilde x}=-\tilde v=0$, and LaSalle's principle gives convergence of that averaged system. To establish convergence of the actual randomly switched system, we also control evolution between refresh times, as follows.

Let $\lambda_2>0$ and $\lambda_N$ be the smallest positive and largest eigenvalues of $L$, respectively, and define
\begin{align}
 b_-&=\min\{1,1/(\alpha\beta\lambda_N)\},\\
 b_+&=\max\{1,1/(\alpha\beta\lambda_2)\},\\
 B&=\alpha\ell_f+\beta\lambda_N.
\end{align}
Choose
\begin{equation}\label{eq:epsilon_choice}
 0<\varepsilon\leq
 \min\left\{\frac{b_-}{2},
     \frac{\alpha m_f}{2\alpha\beta\lambda_N+B^2}\right\}.
\end{equation}
Add a small cross term to \eqref{eq:V_original}:
\begin{equation}\label{eq:V_strict}
 V_\varepsilon=V+\varepsilon\tilde x^\top\tilde v.
\end{equation}
For $\zeta=\operatorname{col}(\tilde x,\tilde v)$, set
\begin{equation}
 \begin{aligned}
 c_-&=b_--\varepsilon,\qquad c_+=b_++\varepsilon,\\
 c_0&=\tfrac12\min\{\alpha m_f,\varepsilon\}.
 \end{aligned}
\end{equation}
Then
\begin{equation}\label{eq:V_bounds}
 \frac{c_-}{2}\|\zeta\|^2
 \leq V_\varepsilon(\zeta)
 \leq\frac{c_+}{2}\|\zeta\|^2.
\end{equation}

To obtain a strict conditional drift bound, the additional cross term has expected derivative
\begin{align}
 &\mathbb E\!\left[\frac{d}{dt}(\tilde x^\top\tilde v)(t_k^+)
                   \,\middle|\,\mathcal F_k\right]\\
 &\quad=-\alpha\tilde v_k^\top h_k
       -\beta\tilde v_k^\top(L\otimes I_d)\tilde x_k\nonumber\\
 &\qquad\quad-\|\tilde v_k\|^2
       +\alpha\beta\tilde x_k^\top(L\otimes I_d)\tilde x_k.\nonumber
\end{align}
Using $\|h_k\|\leq\ell_f\|\tilde x_k\|$ and Young's inequality gives
\begin{align}
 &\mathbb E[\dot V_\varepsilon(t_k^+)\mid\mathcal F_k]\\
 &\quad\leq-\left[\alpha m_f-\varepsilon
          \left(\alpha\beta\lambda_N+\frac{B^2}{2}\right)\right]
            \|\tilde x_k\|^2\nonumber\\
 &\qquad\quad-\frac{\varepsilon}{2}\|\tilde v_k\|^2
 \leq-c_0\|\zeta_k\|^2,\nonumber
\end{align}
where the final inequality follows from \eqref{eq:epsilon_choice}.

Define the direction-dependent Lipschitz bound
\begin{align}\label{eq:C_definition}
 C(u)&=C_0+C_1\|u\|^2,\\
 C_0&=\alpha\ell_f+1,\qquad
 C_1=\beta\sqrt{1+\alpha^2}\lambda_N.\nonumber
\end{align}
Assume that for some $\bar\tau>0$,
\begin{equation}\label{eq:moment_assumption}
 M_{\bar\tau}:=\mathbb E[C(u)^2e^{2\bar\tau C(u)}]<\infty.
\end{equation}
This holds for Rademacher and scaled coordinate vectors for every finite $\bar\tau$. For standard Gaussian vectors, it holds whenever $\bar\tau<1/(4C_1)$.

\begin{thm}\label{thm:convergence}
Under the stated graph, strong convexity, Lipschitz gradient, initialization, and independent sampling assumptions, suppose \eqref{eq:isotropy} and \eqref{eq:moment_assumption} hold. If
\begin{equation}\label{eq:refresh_condition}
 0<\tau\leq\min\left\{\bar\tau,
       \frac{c_0}{2c_+M_{\bar\tau}},\frac{c_+}{2c_0}\right\},
\end{equation}
then \eqref{eq:mod_v}--\eqref{eq:mod_x} converge to $(x^*,v^*)$ in mean square and almost surely. For deterministic initial states and
$r=1-c_0\tau/c_+\in[1/2,1)$,
\begin{equation}\label{eq:mean_square_rate}
 \mathbb E\|\zeta(t_k)\|^2
 \leq\frac{c_+}{c_-}r^k\|\zeta(0)\|^2.
\end{equation}
\end{thm}

\begin{proof}
For a fixed $u$, write the error dynamics as $\dot\zeta=b_u(\zeta)$. The Lipschitz property of the gradients and \eqref{eq:C_definition} give
\begin{equation}
 \|b_u(\zeta)-b_u(\eta)\|\leq C(u)\|\zeta-\eta\|,
 \qquad b_u(0)=0.
\end{equation}
On the current holding interval, for $0\leq s\leq\tau$,
\begin{align}
 \|\zeta(t_k+s)\|&\leq e^{C(u)s}\|\zeta_k\|,\\
 \|\zeta(t_k+s)-\zeta_k\|
       &\leq(e^{C(u)s}-1)\|\zeta_k\|.
\end{align}
Since $V_\varepsilon$ is quadratic and the norm of its symmetric matrix is at most $c_+$, these bounds imply
\begin{align}
 &|\dot V_\varepsilon(t_k+s)-\dot V_\varepsilon(t_k^+)|\\
 &\qquad\leq c_+ C(u)(e^{2C(u)s}-1)\|\zeta_k\|^2.\nonumber
\end{align}
Integrating and using $e^a-1-a\leq a^2e^a/2$ for $a\geq0$, the remainder is bounded by
\begin{align}
 &|V_\varepsilon(t_{k+1})-V_\varepsilon(t_k)
                 -\tau\dot V_\varepsilon(t_k^+)|\\
 &\qquad\leq c_+C(u_k)^2\tau^2e^{2C(u_k)\tau}
                      \|\zeta_k\|^2.\nonumber
\end{align}
Taking conditional expectation, using independence of $u_k$ from $\mathcal F_k$, and applying \eqref{eq:refresh_condition} yields
\begin{align}
 &\mathbb E[V_\varepsilon(t_{k+1})\mid\mathcal F_k]
                     -V_\varepsilon(t_k)\\
 &\quad\leq(-c_0\tau+c_+M_{\bar\tau}\tau^2)\|\zeta_k\|^2\nonumber\\
 &\quad\leq-\frac{c_0\tau}{2}\|\zeta_k\|^2
 \leq-\frac{c_0\tau}{c_+}V_\varepsilon(t_k).\nonumber
\end{align}
Iteration and \eqref{eq:V_bounds} prove \eqref{eq:mean_square_rate}.

The interval bound also gives
\begin{align}
 &\mathbb E\!\left[\sup_{t_k\leq t\leq t_{k+1}}
                           \|\zeta(t)\|^2\right]\\
 &\qquad\leq\mathbb E[e^{2\tau C(u)}]\,
                          \mathbb E\|\zeta_k\|^2.\nonumber
\end{align}
The first factor is finite by \eqref{eq:moment_assumption}, and the right-hand side is geometrically summable in $k$. Thus mean-square convergence holds between refresh times as well. Markov's inequality and the Borel--Cantelli lemma, applied to the interval suprema, imply $\zeta(t)\to0$ almost surely.
\end{proof}

\begin{rem}
The bound \eqref{eq:refresh_condition} is sufficient and conservative. The proof uses the original Lyapunov function together with a small cross term to control the tracking error. Identical second moments give the same initial conditional drift, but the admissible holding interval also depends on higher moments through $M_{\bar\tau}$. This theorem does not assert stability for arbitrary refresh intervals.
\end{rem}

\subsection{Variance and Steady-State Trajectory Fluctuation Analysis}
The preceding analysis guarantees convergence to $z^*$ under an explicit refresh condition. Random encoding still introduces transient fluctuations, whose magnitude can be quantified at the sampling times.

\subsection{Random Differential Equation and Multiplicative Perturbation}
Let $P(t)=I_N\otimes(u_ku_k^\top)$ on $[t_k,t_{k+1})$. Decompose this operator as
\begin{equation}
 P(t)=I_{Nd}+\mathbf\Delta_k,\qquad
 \mathbb E[\mathbf\Delta_k\mid\mathcal F_k]=0.
\end{equation}
Define the coupling perturbation
\begin{equation}
 \xi(t)=(L\otimes I_d)\mathbf\Delta_k\tilde x(t).
\end{equation}
The actual error dynamics can then be written as
\begin{align}\label{eq:error_perturbation}
 \dot{\tilde x}
    &=-\alpha h-\beta(L\otimes I_d)\tilde x
                    -\tilde v-\beta\xi(t),\\
 \dot{\tilde v}
    &=\alpha\beta(L\otimes I_d)\tilde x
                    +\alpha\beta\xi(t).\nonumber
\end{align}
This is a random differential equation with piecewise-constant directions, not an It\^{o} stochastic differential equation. A Brownian diffusion model would require a separate limiting argument. The perturbation is multiplicative in the disagreement and vanishes at consensus; it affects both the state and tracking equations.

\subsection{Quantifying the Projection Variance}
For a fixed vector $a\in\mathbb R^d$, Gaussian fourth moments give
\begin{equation}\label{eq:gauss_variance}
 \mathbb E\|(uu^\top-I_d)a\|^2=(d+1)\|a\|^2.
\end{equation}
Indeed, $\mathbb E[(uu^\top)^2]=(d+2)I_d$ and $\mathbb E[uu^\top]=I_d$. For Rademacher vectors or $u=\sqrt d\,e_J$ with uniform $J$, $\|u\|^2=d$ and $\mathbb E[(uu^\top)^2]=dI_d$, so
\begin{equation}\label{eq:bounded_variance}
 \mathbb E\|(uu^\top-I_d)a\|^2=(d-1)\|a\|^2.
\end{equation}
Consequently, at each refresh time,
\begin{align}
 \mathbb E[\xi(t_k^+)\mid\mathcal F_k]&=0,\\
 \mathbb E[\|\xi(t_k^+)\|^2\mid\mathcal F_k]
   &=\omega\|(L\otimes I_d)\tilde x_k\|^2\nonumber\\
   &\leq\omega\lambda_N^2\|\tilde x_k\|^2,
\end{align}
where $\omega=d+1$ for Gaussian directions and $\omega=d-1$ for Rademacher or scaled coordinate directions. In particular, the variance does not decrease as $1/d$ for these unbiased encoders. These identities concern a fresh direction; independence is not assumed within the holding interval.

\subsection{Steady-State Behavior}
Let $X(t)=\mathbb E[\tilde x(t)\tilde x(t)^\top]$ denote the second-moment matrix of the state error. From Theorem~\ref{thm:convergence},
\begin{equation}
 \lim_{t\to\infty}\operatorname{tr}X(t)
 =\lim_{t\to\infty}\mathbb E\|\tilde x(t)\|^2=0.
\end{equation}
Hence, under the stated assumptions, constant positive gains and sufficiently frequent direction refreshes yield exact convergence; random encoding does not force a nonzero residual error ball. This is consistent with \eqref{eq:error_perturbation}, since the coupling perturbation vanishes when all agents agree.

\begin{rem}
A diminishing coupling gain is not required by this convergence result. The continuous-time proof concerns the specified held-direction model. A discrete-time or sampled-message implementation requires its own step-size and sampling analysis.
\end{rem}
\clearpage


==> intro1.tex <==
\section{Introduction}
\label{sec:introduction}

Distributed optimization enables a network of $N$ agents to
cooperatively solve
\begin{equation}\label{eq:global_opt}
  \min_{z\in\mathbb{R}^{d}} F(z)=\sum\nolimits_{i=1}^{N} f^i(z),
\end{equation}
where each local objective $f^i$ is private to agent~$i$, using
only local computation and neighbor communication. Applications
include cooperative control, distributed estimation, resource
allocation, and networked learning, and the field now offers a
mature set of discrete- and continuous-time algorithms with strong
convergence guarantees, see e.g.,~\cite{nedic2009distributed,qu2017harnessing,kia2019tutorial}.
Consensus provides the basic coordination mechanism: classical
results characterize how graph connectivity and spectral properties
govern agreement, and randomized gossip shows that local randomized
interactions can support distributed
averaging~\cite{olfati2007consensus,boyd2006gossip}. The challenge
in optimization is to combine this agreement mechanism with local
descent so that the common limit minimizes~$F$.

Early distributed subgradient methods established convergence by
combining local subgradient evaluations with information exchange
over the network~\cite{nedic2009distributed}. EXTRA and gradient
tracking subsequently enabled exact convergence with fixed step
sizes~\cite{shi2015extra,nedic2017diging,qu2017harnessing}.
Continuous-time coordination algorithms provide a complementary
perspective in which gradient feedback, consensus coupling, and
integral correction are analyzed with stability tools. In
particular, Kia \emph{et al.}~\cite{SSK-JC-SM:15optim} developed
continuous-time distributed optimization dynamics and studied their
implementation with periodic and event-triggered communication. The
present paper builds on this continuous-time~template.

Despite these mature solution approaches, communication remains a
key impediment for networks of battery-limited or
resource-constrained agents, particularly when the decision variable
is high dimensional ($d\gg 1$) and neighbors exchange full
$d$-dimensional vectors. One line of work reduces the
\emph{frequency} of communication: event- and self-triggered
mechanisms transmit only when a local error exceeds a
threshold~\cite{dimarogonas2012event,seyboth2013event,SSK-JC-SM:15optim},
and randomly activated or time-varying topologies allow agents to
skip rounds. These strategies reduce the number of transmissions,
but each message still carries $\mathcal{O}(d)$~entries.

A second line reduces the \emph{payload} of each message. For
unconstrained distributed optimization over graphs, the effect of
quantized communication on distributed subgradient methods was
first characterized in~\cite{nedic2008quantization}, and subsequent
work established data-rate conditions for
convergence~\cite{yi2014quantized}, quantizer designs tailored to
the optimization dynamics~\cite{pu2017quantization}, and
convergence of gradient methods under limited
communication~\cite{magnusson2018convergence}. Adaptive and dynamic
quantization schemes recover exact convergence with finite
bits~\cite{doan2021fast,reisizadeh2019exact}, including at a linear
rate for smooth, strongly convex
costs~\cite{kajiyama2021linear}. These results build on quantized
consensus, where agreement under restricted precision is analyzed
for deterministic and probabilistic
quantizers~\cite{kashyap2007quantized,carli2010gossip,li2011distributed}.
Similar approaches have been pursued for distributed optimization
in other settings. In distributed learning, QSGD quantifies the
tradeoff between gradient quantization and estimator
variance~\cite{alistarh2017qsgd}, while memory and error-feedback
mechanisms retain information discarded by
compression~\cite{stich2018memory,karimireddy2019error}.
Koloskova \emph{et al.}~\cite{koloskova2019choco} developed
decentralized algorithms in which neighbors exchange quantized or
sparsified model updates, with guarantees for biased and unbiased
compressors; compressed gradient tracking obtains linear
convergence for smooth, strongly convex
objectives~\cite{liao2022compressed}; and robust compressed
push--pull methods extend this direction to directed networks and
nonconvex objectives~\cite{liao2024robust}. Across these methods,
each message still scales with $d$ (at a reduced number of bits per
entry), convergence depends on both the compressor and how it is
integrated into the algorithm, and handling compression error
typically calls for additional error-compensation or tracking
states.

In this paper, we explore a new mechanism for reducing message size
in distributed optimization, inspired by recent federated learning
work that decomposes a vector into a scalar and a random
direction~\cite{rostami2024fedscalar,rostami2026scalar}. For any
random direction $u\in\mathbb{R}^d$ with $\mathbb{E}[uu^\top]=I_d$,
a vector $g\in\mathbb{R}^d$, such as a gradient  update 
satisfies
\begin{equation}
  \nabla f(x)=\mathbb{E}\big[\,\underbrace{u}_{\text{vector}}\,
     \underbrace{u^\top \nabla f(x)}_{\text{scalar}}\,\big].
\end{equation}
Because $u$ can be regenerated from a compact random seed, each
client in~\cite{rostami2024fedscalar,rostami2026scalar} transmits
only the scalar $u^\top \nabla f(x)$ and the seed. The server regenerates $u$
and aggregates the decoded estimates $(u^\top \nabla f(x))\, u$. This reduces
the per-client uplink payload from $\mathcal{O}(d)$ to
$\mathcal{O}(1)$, independently of the model or policy dimension~$d$.

We carry this principle over from client--server aggregation to
neighbor interactions in continuous-time, consensus-based
distributed optimization, where the encoded quantities are the
exchanged state vectors rather than gradients. All agents regenerate
a common direction $u_k\in\mathbb{R}^d$ at refresh times $t_k=k\tau$
from a shared seed and synchronized index, so no seed needs to be
transmitted. Agent~$i$ sends the scalar $c^i(t)=u_k^\top x^i(t)$,
and its neighbors decode $u_k c^i(t)$ to form the coupling
$u_k u_k^\top\big(x^i(t)-x^j(t)\big)$. Each agent still uses its
full local gradient $\nabla f^i(x^i(t))$. Each neighbor exchange
therefore carries one real number instead of a $d$-dimensional
state, and the scheme needs neither transmission of the direction
vector nor compression-error memory. Our continuous-time model
retains a continuously varying scalar signal within each
direction-holding interval; sampling and finite-bit quantization are
separate implementation considerations.

The framework admits any direction distribution satisfying isotropy,
$\mathbb{E}[u_k u_k^\top]=I_d$, and a stated exponential-moment
condition, with independent draws across refreshes. Gaussian and
Rademacher directions are admissible, and uniform coordinate
communication is included by choosing $u_k=\sqrt{d}\,e_{J_k}$ with
$J_k$ uniform on $\{1,\ldots,d\}$. This flexibility lets the
direction choice reflect the geometry of the disagreement. When
disagreement energy is spread evenly across coordinates, coordinate
sampling exposes a comparable amount of disagreement at each
selection. When disagreement is concentrated in a few coordinates,
most coordinate selections miss the active components, whereas
dense Gaussian or Rademacher directions mix them into every
transmitted scalar and can improve transient behavior. These effects
depend on the disagreement structure and do not imply a universal
ordering of expected convergence rates.

The analysis must account for the interaction between random
communication and the coupled state and integral dynamics. Although
the encoder is unbiased at each refresh, holding a direction over a
nonzero interval creates dependence between that direction and the
evolving network state. We control this dependence by combining
conditional Lyapunov drift at refresh times with bounds on the
intervening evolution. Our contributions are threefold. First, we
show that the common optimal equilibrium is preserved and is unique
on the zero-sum integral-state subspace. Second, for strongly convex
local objectives with globally Lipschitz gradients and constant
positive gains, we establish exponential mean-square and almost-sure
convergence to the optimizer under an explicit upper bound on the
refresh interval; this bound makes the roles of graph connectivity,
objective regularity, and direction statistics explicit. Third, we
derive distribution-dependent encoding-variance identities for
Gaussian, Rademacher, and scaled coordinate directions. Together,
these results show that scalar communication preserves exact
convergence to the optimizer. Although we develop the mechanism in
continuous time, the scalar encoding principle extends naturally to
discrete-time updates, quantized communication, and other
distributed optimization architectures.


==> intro2.tex <==
\section{Introduction}
\label{sec:introduction}

Distributed optimization enables a network of $N$ agents to
cooperatively solve
\begin{equation}\label{eq:global_opt}
  \min_{z\in\mathbb{R}^{d}} F(z)=\sum\nolimits_{i=1}^{N} f^i(z),
\end{equation}
where each local objective $f^i$ is private to agent~$i$, using
only local computation and communication with neighbors. Problems
of this form arise in cooperative control, distributed estimation,
resource allocation, and networked learning, and the field now
offers a mature set of discrete- and continuous-time algorithms with
strong convergence guarantees; see,
e.g.,~\cite{nedic2009distributed,qu2017harnessing,nedic2018distributed,yang2019survey}.

Despite these advances, communication remains a key impediment to deploying distributed optimization algorithms on resource-constrained networks. Two aspects of communication cost are particularly important. The first is \emph{energy}: in battery-powered systems, every transmission depletes a limited energy budget, motivating methods that reduce how often agents communicate. The second is \emph{bandwidth}: communication channels limit how much information can be carried by a single message, motivating methods that reduce the size of each transmission. While both constraints are important, they call for fundamentally different remedies. Event- and self-triggered mechanisms~\cite{dimarogonas2012event,seyboth2013event,SSK-JC-SM:15optim} primarily address the energy side by reducing communication frequency. However, each transmitted message still typically contains a full $d$-dimensional state or gradient vector, resulting in a per-message communication cost that scales with $d$. Quantization and sparsification reduce the number of transmitted bits or entries, but the exchanged objects remain $d$-dimensional and often require auxiliary error-compensation or tracking mechanisms. The bandwidth burden is particularly significant in high-dimensional problems. It also arises in challenging communication environments with packet loss, noise, or intermittent connectivity, where improving reliability may require retransmissions or communication redundancy. In such settings, smaller messages provide greater flexibility within a fixed bandwidth budget. These considerations motivate distributed optimization algorithms whose per-message communication cost is independent of the decision~dimension. 

To achieve dimension-independent communication, we pursue a scalar encoding strategy that reduces each neighbor message to a single real number, independent of~$d$. The idea originates in our recent federated learning work~\cite{rostami2024fedscalar,rostami2026scalar}: for any random
direction $u\in\mathbb{R}^d$ with $\mathbb{E}[uu^\top]=I_d$, a
vector $g\in\mathbb{R}^d$ satisfies
\begin{equation}\label{eq:decomposition}
  g=\mathbb{E}\big[\,\underbrace{u}_{\text{vector}}\,
     \underbrace{u^\top g}_{\text{scalar}}\,\big],
\end{equation}
so a client that shares a random seed with the server need only
transmit the scalar $u^\top g$; the server regenerates $u$ and
aggregates the decoded estimates $(u^\top g)\,u$ of local model
updates. We carry this principle from client--server aggregation to
neighbor interactions in consensus-based distributed optimization,
where the encoded quantities are the exchanged states. All agents
regenerate a common direction $u_k$ at refresh times $t_k=k\tau$
from a shared seed, agent~$i$ sends the scalar
$c^i(t)=u_k^\top x^i(t)$, and its neighbors decode $c^i(t)\,u_k$ to
form the rank-one coupling $u_ku_k^\top(x^i-x^j)$, while every agent
keeps using its full local gradient. No direction vector is
transmitted and no compression-error memory is needed. We develop
the mechanism in continuous time on the coordination algorithm
of~\cite{SSK-JC-SM:15optim}, but it applies equally to any
distributed optimization algorithm whose inter-agent coupling
depends only on relative states, and its scalar encoding principle
extends to discrete-time updates and quantized communication.

\emph{Contributions:} We propose a scalar-communication
distributed optimization algorithm in which neighbors exchange one
real number per message. Our analysis must account for the
interaction between random communication and the coupled state and
integral dynamics: although the encoder is unbiased at each refresh,
holding a direction over a nonzero interval creates dependence
between that direction and the evolving network state. We control
this dependence by combining conditional Lyapunov drift at refresh
times with bounds on the intervening evolution. Our results are
threefold. First, we show that the optimal consensus equilibrium is
preserved and is unique on the zero-sum integral-state subspace.
Second, for strongly convex local objectives with globally Lipschitz
gradients and constant gains, we establish exponential mean-square
and almost-sure convergence to the optimizer under an explicit upper
bound on the refresh interval, which makes the roles of graph
connectivity, objective regularity, and direction statistics
explicit. Third, we derive encoding-variance identities for
Gaussian, Rademacher, and scaled coordinate directions, the last of
which recovers random coordinate communication as a special case.
The framework admits any isotropic direction distribution satisfying
a stated moment condition, which lets the direction choice reflect
the structure of the disagreement: coordinate directions expose one
entry at a time, whereas dense Rademacher or Gaussian directions mix
all entries into every transmitted scalar.

\emph{Literature review:} Early distributed subgradient methods
combine local subgradient steps with network
averaging~\cite{nedic2009distributed}, and EXTRA and gradient
tracking later achieved exact convergence with fixed step
sizes~\cite{shi2015extra,nedic2017diging,qu2017harnessing}.
Continuous-time algorithms offer a complementary view in which
gradient feedback, consensus coupling, and integral correction are
analyzed with stability tools~\cite{wang2010control,wang2011control,gharesifard2014distributed,SSK-JC-SM:15optim}.
For unconstrained distributed optimization over graphs, the effect
of quantized communication on subgradient methods was first
characterized in~\cite{nedic2008quantization}; subsequent work
established data-rate conditions~\cite{yi2014quantized}, quantizer
designs tailored to the optimization
dynamics~\cite{pu2017quantization}, and convergence under limited
communication~\cite{magnusson2018convergence}, while adaptive
quantization recovers exact convergence with finite
bits~\cite{doan2021fast,reisizadeh2019exact}, including at a linear
rate for smooth, strongly convex costs~\cite{kajiyama2021linear}.
These results build on quantized
consensus~\cite{kashyap2007quantized,carli2010gossip,li2011distributed}.
Similar approaches have been pursued in distributed learning:
QSGD quantifies the tradeoff between gradient quantization and
estimator variance~\cite{alistarh2017qsgd}; memory and
error-feedback mechanisms retain information discarded by
compression~\cite{stich2018memory,karimireddy2019error};
Koloskova \emph{et al.}~\cite{koloskova2019choco} analyze
decentralized methods with quantized or sparsified updates under
biased and unbiased compressors; and compressed gradient tracking
and push--pull methods obtain linear convergence and extend to
directed networks and nonconvex
objectives~\cite{liao2022compressed,liao2024robust}.

\emph{Organization:} Section~\ref{sec:problem} states the problem
and the baseline algorithm. Section~\ref{sec:scalar} introduces the
scalar encoding, verifies that the optimizer remains the unique
equilibrium, shows why a fixed direction fails, and establishes
convergence under direction refreshing together with the encoding
variance analysis. Section~\ref{sec:numerical} presents a numerical
example, and Section~\ref{sec:conclusion} concludes.

==> numerical0.tex <==
\section{Numerical Example}
\label{sec:numerical}

We consider $20$ agents with $64$-dimensional states solving
$\min_x \frac{1}{20}\sum_{i=1}^{20}f^i(x)$ over a connected
undirected network. The agents are arranged on a ring, and
each agent is connected to the agents one, four, and seven
positions away in both directions. Thus, every agent has six
neighbors, and the graph has $60$ edges. We scale the
Laplacian so that $\lambda_{\max}(L)=1$. The local costs are
\[
f^i(x)=\frac12 z^\top H z
+0.06\sum\nolimits_{j=1}^{64}\log\cosh(z_j)-b_i^\top z,
\]
where $z=x-c$, $c=10e_1$,
$H=\operatorname{diag}(1,0.3,1,\ldots,1)$, and
$b_i=(s_i-\bar s)e_2$. The variables $s_i$ independently
take values $\pm1$ with equal probability, and
$\bar s=20^{-1}\sum_i s_i$. These functions are strongly
convex with globally Lipschitz gradients, since
$0.3I\preceq\nabla^2f^i(x)\preceq1.06I$.
Their aggregate minimizer is $x^\star=c$.
We initialize $x_i^0=c+b_i$ and $v_i^0=0$: agents initially
agree on the large first coordinate but disagree on the
second coordinate.

We discretize the proposed dynamics using simultaneous
forward-Euler updates with unit gains. The proposed scheme,
denoted \emph{ScalarCom}, uses either uniform coordinate
directions $u_k=\sqrt{64}\,e_{J_k}$ or independent Rademacher
entries. A fresh direction is generated by the agents from prefixed common seed by all agents each
round. We compare these variants with full-vector exchange,
Top-1, QSGD with $s=1$, and scaled sign encoding. All methods
retain full local gradients and encode current states
without error feedback.

For every method, we test the same constant step-size grid:
\[
\begin{split}
\mathcal H=\{&
0.004,0.008,0.012,0.016,0.020,0.024,0.028,\\
&0.032,0.06,0.125,0.25,0.5,1\}.
\end{split}
\]
Each candidate is evaluated for $2500$ rounds on two
training instances, with eight random trials per stochastic
method and instance. We discard candidates producing
nonfinite errors or a relative error of at least $100$,
and select the remaining step with the smallest RMS error
at a total communication budget of $7.2$ Mbit. The selected
steps are $0.020$ for coordinate ScalarCom, $0.024$ for
Rademacher ScalarCom, $1$ for full-vector exchange,
$0.004$ for Top-1, $0.008$ for QSGD, and $0.032$ for
Sign method. These steps are then fixed for evaluation
on three new problem instances, using $24$ random trials
per stochastic method and instance.

The plotted error measures how far the agents remain
from the optimizer relative to their initial distance.
For each run, we compute
\[
r_k=
\left(
\frac{\sum_{i=1}^{20}\|x_i^k-x^\star\|^2}
{\sum_{i=1}^{20}\|x_i^0-x^\star\|^2}
\right)^{1/2}.
\]
We then square $r_k$, average across runs, and take the
square root to obtain the reported root-mean-square
(RMS) relative distance. Thus, the curves start at one,
and smaller values indicate greater accuracy.
Communication counts payload bits transmitted across
all network links, including indices, scales, and seed
initialization. Each ScalarCom message uses $32$ bits,
compared with $38$ for Top-1, $96$ for Sign method,
and $2048$ for full-vector exchange. QSGD uses a
variable-length representation; protocol headers
are excluded uniformly.

Figure~\ref{fig:numerical} shows that full-vector exchange
requires the fewest rounds, but its larger messages
increase communication cost. At $7.2$ Mbit, Rademacher
ScalarCom achieves an RMS relative error of
$7.43\times10^{-6}$, compared with $7.63\times10^{-4}$
for coordinate ScalarCom and $1.56\times10^{-3}$ for
full-vector exchange. With the same step $h=0.020$
for both scalar variants, Rademacher still achieves
approximately $47$ times lower RMS error. This result
reflects the effect of slow coordinate-sampling
trajectories on mean-square performance; coordinate
sampling has a lower median error at this budget.

The example also illustrates the benefit of shared
linear encoding: the common state component cancels
from its ideal consensus feedback because
$L(X+\mathbf1_n c^\top)uu^\top=LXuu^\top$.
Top-1 instead repeatedly selects the already-agreed
large coordinate, while coarse quantization can
poorly represent smaller informative differences.
The observed advantages concern this constructed
problem and finite communication budgets, rather
than a universal ordering of compression methods.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.34]
    {Fig/02_optimization_comparison.pdf}
    \caption{RMS relative distance to the optimizer
    versus communication rounds (left) and total
    network communication (right). Lower is better.
    Full-vector exchange is faster in rounds,
    whereas scalar encoding uses fewer bits to
    attain the reported accuracy. The dotted line
    marks a relative error of $10^{-3}$.}
    \label{fig:numerical}
\end{figure}



==> numerical_example_v2.tex <==
\section{Numerical Example}
\label{sec:numerical}

We study distributed $\ell_2$-regularized logistic regression with
$N=20$ agents, $d=64$, and
\begin{equation}
 f^i(x)=\frac{1}{m}\sum_{s=1}^{m}
 \log\!\left(1+e^{-y_{i,s}a_{i,s}^{\top}x}\right)
 +\frac{0.3}{2}\|x\|^2 .
\end{equation}
The synthetic data are constructed to isolate the interaction between
direction selection and objective curvature. Each agent has $128$
observations of each feature $\gamma_j e_j$, giving $m=8192$ samples,
where $\gamma_j=16$ for $j\le49$ and $\gamma_j=2$ otherwise.
The resulting local costs satisfy Assumption~\ref{assump:cost} with
$m_f=0.3$ and $\ell_f\le1.3$. Agents form a cycle, with each agent
connected to its first and third neighbors in both directions; every
edge has weight $1/8$. We use $\alpha=\beta=1$ and
$x^i(0)=v^i(0)=0$ throughout.

The two client populations alternate around the cycle. Both have a
positive-label proportion of $3/4$ for feature~1. In the
\emph{concentrated} case, the positive-label proportions for feature~50
are $1/8$ and $7/8$, respectively, and all other features are balanced.
In the \emph{spread} case, the proportions are $1/2-1/128$ and
$1/2+1/128$ for features~2--37, with the remaining features balanced.
The two cases have exactly the same aggregate objective and minimizer
$z^\star$, and the same local gradient-heterogeneity norm $3/256$.
Only its alignment changes: it occupies one weak-curvature coordinate
or 36 stronger-curvature coordinates. The minimizer is computed
centrally for evaluation, with gradient residual below $10^{-12}$.

We integrate the continuous-time dynamics using fourth-order
Runge--Kutta steps that end at every direction refresh. The maximum
integration step is $0.4/(d+1.3)$, with at least four steps per holding
interval; this numerical step is distinct from $\tau$. All encoders
use the same integration rule and gains. A same-stream check with
the actual integration step halved changes the reported RMS curves
by less than $0.2\%$ in the verification runs. We compare shared
Rademacher directions, shared uniform scaled-coordinate directions,
and full-vector exchange. For $M$ independent direction sequences,
we report
\begin{equation}
 E_{\mathrm{RMS}}(t)=
 \left(\frac{\sum_{r=1}^{M}\sum_{i=1}^{N}
 \|x_r^i(t)-z^\star\|^2}{MN\|z^\star\|^2}\right)^{1/2}.
\end{equation}
Thus, $E_{\mathrm{RMS}}(0)=1$, and $10^{-3}$ represents $0.1\%$
of the initial root-mean-square distance.

Figure~\ref{fig:geometry} uses $\tau=2/64$ and $4096$ independent
direction sequences per stochastic method. At $t=20$, Rademacher
encoding attains an empirical RMS error of $0.00504$, compared with
$0.0760$ for coordinate encoding in the concentrated case. In the
spread case, coordinate encoding attains $0.00245$, compared with
$0.00414$ for Rademacher encoding. These comparisons concern
mean-square performance: coordinate encoding can have a smaller
median error while exhibiting rare, much slower trajectories.
The reversal depends on curvature alignment, rather than sparsity
alone. Coordinate feedback preserves the active coordinate subspace;
dense feedback transfers disagreement between coordinates of different
curvature. This can help when the active direction has weak curvature
and hurt when the active subspace already has stronger curvature.
The theorem supplies a common sufficient guarantee for both encoders,
without imposing a universal performance ordering.

Figure~\ref{fig:refresh} examines the concentrated case as $\tau$
varies. Frequent refreshing yields rapid decay, whereas longer
holding intervals leave larger finite-horizon errors. A fixed direction
leaves persistent error, consistent with the frozen-direction
equilibria discussed earlier. The tested intervals exceed the
conservative sufficient bound, so these observations do not identify
a necessary stability threshold or an optimal $\tau$. The scalar
methods communicate one continuously varying real-valued signal per
link, compared with 64 for full-vector exchange; these continuous-time
experiments do not establish a total-bit communication complexity.

\begin{figure*}[t]
 \centering
 \includegraphics[width=\textwidth]{fig/fig_geometry.pdf}
 \caption{Controlled logistic-regression comparison at $d\tau=2$.
 Both cases share the aggregate objective, optimizer, graph, gains,
 initialization, and gradient-heterogeneity norm. Curves show empirical
 RMS error over 4096 direction sequences; bands are pointwise 95\%
 bootstrap intervals for the RMS estimate. The left case concentrates
 heterogeneity in a weak-curvature coordinate; the right spreads it
 across 36 stronger-curvature coordinates.}
 \label{fig:geometry}
 \label{fig:rvc}
\end{figure*}

\begin{figure*}[t]
 \centering
 \includegraphics[width=\textwidth]{fig/fig_refresh.pdf}
 \caption{Effect of the holding interval in the concentrated case.
 (a) Rademacher trajectories at several $d\tau$, with full-vector and
 fixed-direction references. (b) Empirical RMS error at $t=40$ versus
 $d\tau$ for both encoders. The sweep uses 128 direction sequences
 per point, except $d\tau=2$, which reuses the 4096-sequence comparison;
 error bars are pointwise 95\% bootstrap intervals. Finite-horizon
 errors and uncertainty do not establish an instability threshold.}
 \label{fig:refresh}
 \label{fig:ct}
\end{figure*}


==> technical0.tex <==
\subsection{Convergence under Direction Refreshing}
\label{subsec:convergence}
Let $u_k$ be redrawn independently from a fixed distribution at the
refresh times $t_k=k\tau$. We derive a sufficient upper bound on
$\tau$; unbiasedness alone does not guarantee convergence for
arbitrary holding intervals.

Let $\mathcal F_k$ denote the history immediately before drawing
$u_k$, and assume
\begin{equation}\label{eq:isotropy}
    \mathbb E[u_ku_k^\top\mid\mathcal F_k]=I_d,
\end{equation}
which holds for all three distributions (G), (R), and (C). At a
refresh time, the states are $\mathcal F_k$-measurable, so
\begin{align}
 \mathbb E[y^i(t_k^+)-y^j(t_k^+)\mid\mathcal F_k]
 &=\mathbb E[u_ku_k^\top\mid\mathcal F_k]\,(x^i(t_k)-x^j(t_k))\nonumber\\
 &=x^i(t_k)-x^j(t_k).
\end{align}
Within a holding interval, however, the states depend on the sampled
direction, so this factorization is available only at refresh
times. A sufficiently small holding interval keeps the resulting
state--direction dependence under control.

Let $x=\operatorname{col}(x^1,\ldots,x^N)$ and define the stacked
cost $G(x)=\sum_{i=1}^N f^i(x^i)$, whose gradient stacks the local
gradients (in contrast to the common-argument cost $F$ in
\eqref{eq:global_opt}). Let
\begin{equation}
    x^\star=\mathbf1_N\otimes z^\star,\qquad
    v^\star=-\alpha\nabla G(x^\star),
\end{equation}
and define the errors $\tilde x=x-x^\star$, $\tilde v=v-v^\star$.
Consider the quadratic Lyapunov candidate
\begin{equation}\label{eq:V_original}
 V=\frac12\tilde x^\top\tilde x
    +\frac1{2\alpha\beta}\tilde v^\top
          (L^\dagger\otimes I_d)\tilde v,
\end{equation}
where $L^\dagger$ is the Moore--Penrose pseudoinverse. Since
$\sum_i\tilde v^i=0$, $V$ is positive definite on the invariant
zero-sum subspace.

Set $h=\nabla G(x)-\nabla G(x^\star)$ and $P=u_ku_k^\top$ on the
current interval. Along \eqref{eq:mod},
\begin{align}\label{eq:actual_V_dot}
 \dot V={}&-\alpha\tilde x^\top h
       -\beta\tilde x^\top(L\otimes P)\tilde x\nonumber\\
     &+\tilde v^\top[I_N\otimes(P-I_d)]\tilde x,
\end{align}
where we used $\tilde v^\top(L^\dagger L\otimes P)
=\tilde v^\top(I_N\otimes P)$, a consequence of the zero-sum
condition. Taking conditional expectation at a refresh time,
\begin{align}\label{eq:mean_V_dot}
 \mathbb E[\dot V(t_k^+)\mid\mathcal F_k]
   ={}&-\alpha\tilde x_k^\top h_k
      -\beta\tilde x_k^\top(L\otimes I_d)\tilde x_k\nonumber\\
   \leq{}&-\alpha m_f\|\tilde x_k\|^2 ,
\end{align}
so the cross terms in $\tilde v$ cancel in expectation. For the
deterministic averaged dynamics (obtained by replacing $P$ with
$I_d$), the same calculation holds at all times; on $\{\tilde x=0\}$
invariance requires $\dot{\tilde x}=-\tilde v=0$, and LaSalle's
principle yields convergence of the averaged system. For the actual
randomly switched system we must also control the evolution between
refresh times.

Let $\lambda_2>0$ and $\lambda_N$ be the smallest positive and
largest eigenvalues of $L$, and define
\begin{align}
 b_-&=\min\{1,1/(\alpha\beta\lambda_N)\},\qquad
 b_+=\max\{1,1/(\alpha\beta\lambda_2)\},\nonumber\\
 B&=\alpha\ell_f+\beta\lambda_N .
\end{align}
Choose
\begin{equation}\label{eq:epsilon_choice}
 0<\varepsilon\leq
 \min\left\{\frac{b_-}{2},
     \frac{\alpha m_f}{2\alpha\beta\lambda_N+B^2}\right\}
\end{equation}
and add a cross term to \eqref{eq:V_original}:
\begin{equation}\label{eq:V_strict}
 V_\varepsilon=V+\varepsilon\tilde x^\top\tilde v .
\end{equation}
For $\zeta=\operatorname{col}(\tilde x,\tilde v)$, set
$c_-=b_--\varepsilon$, $c_+=b_++\varepsilon$, and
$c_0=\tfrac12\min\{\alpha m_f,\varepsilon\}$. Then
\begin{equation}\label{eq:V_bounds}
 \frac{c_-}{2}\|\zeta\|^2
 \leq V_\varepsilon(\zeta)
 \leq\frac{c_+}{2}\|\zeta\|^2 .
\end{equation}
The cross term has expected derivative
\begin{align}
 &\mathbb E\!\left[\frac{d}{dt}(\tilde x^\top\tilde v)(t_k^+)
                   \,\middle|\,\mathcal F_k\right]
  =-\alpha\tilde v_k^\top h_k
       -\beta\tilde v_k^\top(L\otimes I_d)\tilde x_k\nonumber\\
 &\qquad\qquad-\|\tilde v_k\|^2
       +\alpha\beta\tilde x_k^\top(L\otimes I_d)\tilde x_k ,
\end{align}
and using $\|h_k\|\leq\ell_f\|\tilde x_k\|$ with Young's inequality,
\begin{align}\label{eq:strict_drift}
 \mathbb E[\dot V_\varepsilon(t_k^+)\mid\mathcal F_k]
 &\leq-\left[\alpha m_f-\varepsilon
          \left(\alpha\beta\lambda_N+\frac{B^2}{2}\right)\right]
            \|\tilde x_k\|^2\nonumber\\
 &\qquad-\frac{\varepsilon}{2}\|\tilde v_k\|^2
 \;\leq\;-c_0\|\zeta_k\|^2,
\end{align}
where the last inequality follows from \eqref{eq:epsilon_choice}.

To control the evolution within a holding interval, define the
direction-dependent Lipschitz constant
\begin{align}\label{eq:C_definition}
 C(u)&=C_0+C_1\|u\|^2,\\
 C_0&=\alpha\ell_f+1,\qquad
 C_1=\beta\sqrt{1+\alpha^2}\,\lambda_N,\nonumber
\end{align}
and assume that for some $\bar\tau>0$,
\begin{equation}\label{eq:moment_assumption}
 M_{\bar\tau}:=\mathbb E\big[C(u)^2e^{2\bar\tau C(u)}\big]<\infty .
\end{equation}
For the bounded directions (R) and (C), $\|u\|^2=d$, so
$C(u)\equiv C_d:=C_0+C_1d$ is deterministic and
\eqref{eq:moment_assumption} holds for every finite $\bar\tau$ with
$M_{\bar\tau}=C_d^2e^{2\bar\tau C_d}$. For Gaussian directions,
$\|u\|^2$ is chi-square with $d$ degrees of freedom and
\eqref{eq:moment_assumption} holds only for $\bar\tau<1/(4C_1)$.

\begin{thm}\label{thm:convergence}
Let Assumption~\ref{assump:cost} hold, let $\mathcal G$ be connected
and undirected, let $\sum_i v^i(0)=0$, and let the directions $u_k$
be drawn independently across refreshes so that
\eqref{eq:isotropy} and \eqref{eq:moment_assumption} hold. If
\begin{equation}\label{eq:refresh_condition}
 0<\tau\leq\min\left\{\bar\tau,
       \frac{c_0}{2c_+M_{\bar\tau}},\frac{c_+}{2c_0}\right\},
\end{equation}
then the trajectories of \eqref{eq:mod_v}--\eqref{eq:mod_x} converge
to $(x^\star,v^\star)$ in mean square and almost surely. Moreover,
for deterministic initial states and
$r=1-c_0\tau/c_+\in[1/2,1)$,
\begin{equation}\label{eq:mean_square_rate}
 \mathbb E\|\zeta(t_k)\|^2
 \leq\frac{c_+}{c_-}\,r^k\,\|\zeta(0)\|^2 .
\end{equation}
\end{thm}

\begin{proof}
For fixed $u$, write the error dynamics as $\dot\zeta=b_u(\zeta)$.
The Lipschitz property of the gradients and \eqref{eq:C_definition}
give
\begin{equation}
 \|b_u(\zeta)-b_u(\eta)\|\leq C(u)\|\zeta-\eta\|,
 \qquad b_u(0)=0 .
\end{equation}
Hence, on the current holding interval and for $0\leq s\leq\tau$,
\begin{equation}
 \|\zeta(t_k+s)\|\leq e^{C(u)s}\|\zeta_k\|,\qquad
 \|\zeta(t_k+s)-\zeta_k\|\leq(e^{C(u)s}-1)\|\zeta_k\| .
\end{equation}
Since $V_\varepsilon$ is quadratic with symmetric matrix of norm at
most $c_+$, these bounds imply
\begin{equation}
 |\dot V_\varepsilon(t_k+s)-\dot V_\varepsilon(t_k^+)|
 \leq c_+ C(u)\big(e^{2C(u)s}-1\big)\|\zeta_k\|^2 .
\end{equation}
Integrating over $[0,\tau]$ and using $e^a-1-a\leq a^2e^a/2$ for
$a\geq0$,
\begin{equation}
 \big|V_\varepsilon(t_{k+1})-V_\varepsilon(t_k)
      -\tau\dot V_\varepsilon(t_k^+)\big|
 \leq c_+C(u_k)^2\tau^2e^{2C(u_k)\tau}\|\zeta_k\|^2 .
\end{equation}
Taking conditional expectation, using the independence of $u_k$ from
$\mathcal F_k$, \eqref{eq:strict_drift}, and
\eqref{eq:refresh_condition},
\begin{align}
 \mathbb E[V_\varepsilon(t_{k+1})\mid\mathcal F_k]-V_\varepsilon(t_k)
 &\leq(-c_0\tau+c_+M_{\bar\tau}\tau^2)\|\zeta_k\|^2\nonumber\\
 &\leq-\frac{c_0\tau}{2}\|\zeta_k\|^2
 \leq-\frac{c_0\tau}{c_+}V_\varepsilon(t_k).
\end{align}
Iterating and applying \eqref{eq:V_bounds} proves
\eqref{eq:mean_square_rate}.

The interval bound also gives
\begin{equation}
 \mathbb E\!\Big[\sup_{t_k\leq t\leq t_{k+1}}\|\zeta(t)\|^2\Big]
 \leq\mathbb E\big[e^{2\tau C(u)}\big]\,\mathbb E\|\zeta_k\|^2 .
\end{equation}
The first factor is finite by \eqref{eq:moment_assumption} and the
right-hand side is geometrically summable in $k$, so mean-square
convergence holds between refresh times as well. Markov's inequality
and the Borel--Cantelli lemma applied to the interval suprema give
$\zeta(t)\to0$ almost surely.
\end{proof}

\begin{rem}[Rademacher and coordinate directions]
For (R) and (C), $C(u)\equiv C_d$ is deterministic, so one may take
$\bar\tau=\tau$ in \eqref{eq:moment_assumption} and
\eqref{eq:refresh_condition} reduces to the explicit scalar
condition
\begin{equation}
 \tau\leq\min\Big\{\frac{c_0}{2c_+C_d^2e^{2C_d\tau}},
                   \frac{c_+}{2c_0}\Big\},
\end{equation}
which has a nonempty solution set since the right-hand side is
positive at $\tau=0$. No restriction of the form
$\bar\tau<1/(4C_1)$ arises, in contrast to the Gaussian case.
\end{rem}

\begin{rem}[Conservativeness]
The bound \eqref{eq:refresh_condition} is sufficient and
conservative. Distributions with identical second moments produce
the same conditional drift \eqref{eq:strict_drift}, but the
admissible holding interval also depends on higher moments through
$M_{\bar\tau}$. The theorem does not assert stability for arbitrary
refresh intervals.
\end{rem}

